A Specification Logic for Programs in the Probabilistic Guarded Command Language (Extended Version)

The semantics of probabilistic languages has been extensively studied, but specification languages for their properties have received little attention. This paper introduces the probabilistic dynamic logic pDL, a specification logic for programs in the probabilistic guarded command language (pGCL) of McIver and Morgan. The proposed logic pDL can express both first-order state properties and probabilistic reachability properties, addressing both the non-deterministic and probabilistic choice operators of pGCL. In order to precisely explain the meaning of specifications, we formally define the satisfaction relation for pDL. Since pDL embeds pGCL programs in its box-modality operator, pDL satisfiability builds on a formal MDP semantics for pGCL programs. The satisfaction relation is modeled after PCTL, but extended from propositional to first-order setting of dynamic logic, and also embedding program fragments. We study basic properties of pDL, such as weakening and distribution, that can support reasoning systems. Finally, we demonstrate the use of pDL to reason about program behavior.

==> entailment.tex <==
\noindent
We now formalize the intuition that a formula probabilistically entails another, i.e., there is a bound between the expectation that a formula $\phi_2$ holds and the expectation that another formula $\phi_1$ holds.

\begin{definition}[p-Entailment for
  p-Box Formulas] \label{def:p-entail} Let $s_1,s_2\in \pGCL$,
  $\phi_1, \phi_2\in\PDL$, $\pfun,\pfun_1,\pfun_2 \in \State \rightarrow [0,1]$ be
  expectations, and $\epsilon$ be a valuation.  The
  \emph{$p$-entailment} of a p-box formula $[s_2]_{\pfun_2}\phi_2$
  from a p-box  formula $[s_1]_{\pfun_2} \phi_1$,
  denoted $[s_1]_{\pfun_2} \phi_1\models_\pfun [s_2]_{\pfun_2}\phi_2$, is defined by
  $$\begin{array}{l} [s_1]_{\pfun_1} \phi_1\models [s_2]_{\pfun_2} \phi_2\textnormal{
    iff }\\ \qquad \textnormal{for every } \epsilon \textnormal{ such that }\epsilon\models [s_1]_{\pfun_1} \phi_1
  \textnormal{ then } \epsilon \models [s_2]_{\pfun_2}
      \phi_2 \textnormal{ and }  \pfun \cdot \pfun_1 \leq  \pfun_2\enspace. \end{array}$$
\end{definition}
% \pfun\leq  \frac{\pfun_2}{\pfun_1}
% \begin{definition}[$p$-Entailment for DL-Formulas]  \label{def:p-entail}
%   Let $\phi_1, \phi_2\in\PDL$,  $p,p_1,p_2 \in \State \rightarrow [0,1]$ be expectations, and $\epsilon$ range over
%   valuations (states).  The \emph{$p$-entailment} of a formula
%   $\phi_2$ from a formula $\phi_1$, denoted
%   $\phi_1\models_p \phi_2$, is defined by
%   $$\phi_1\models_p \phi_2\textnormal{ iff } \forall \epsilon\; . \;\epsilon\models_{p_1} \phi_1
%   \textnormal{ and } \epsilon \models_{p_2} \phi_2 \textnormal{ implies } p\leq  \frac{p_2}{p_1}.$$
%   \color{gray}
%   $$[s_1]_{p_1} \phi_1\models [s_2]_{p_2} \phi_2\textnormal{ iff } \textnormal{whenever } . \;\epsilon\models [s_1]_{p_1} \phi_1
%   \textnormal{ then } \epsilon \models [s_2]_{p_2} \phi_2\enspace.$$
% \end{definition}
The notion of p-entailment generalises to unboxed formulas by simply
taking their characteristic function as their probability
functions. If $\pfun_1 > 0$ for all $\epsilon$, we can see
p-entailment as expressing a bound between the expectations of the two
formulae, i.e., $p\leq \frac{p_2}{p_1}$.  Furthermore, p-entailment is
a generalization of classical Boolean entailment, in the sense that
for $p = 1$ we have
$$\phi_1\models \phi_2\textnormal{ iff } \forall
\epsilon. \epsilon\models_{p_1} \phi_1 \textnormal{ and } \epsilon
\models_{p_2} \phi_2 \textnormal{ implies } p_1(\epsilon) \leq p_2
(\epsilon)\enspace.$$

\awnote{if we have not theorems about entailment, perhaps drop or move next to validity}

A note to future us: The above is just syntactic sugar for usual implication that is directly derivable from the new definition of satisfaction (could be introduced as such together with disjunction).  Here we may need a  tighter relation between the two programs or two formulae (something that smells some kind of probabilistic (bi-)simulation).

% The use of Expectation macro in this example is broken, needs to be recovered if we want to use this
\begin{example}
  Let $\phi$ be a formula such that $x$ does not occur in $\phi$ and
  let $x:=1 \pchoice{p} x:=0$ be a program which executes $x:=1$ with
  some probability $p$. We have that
$$\phi \models_p [x:=1 \pchoice{p} x:=0] (x==1 \land \phi).$$
To see that this holds, consider the MDP $\MDP$, some valuation
$\epsilon$ and an expectation $p_2$ such that
$$\begin{array}{l}
\charfun{[x:=1 \pchoice{p} x:=0] (x==1 \land \phi)}\\
\qquad =
\Expectation\epsilon{\langle\epsilon,x:=1 \pchoice{p} x:=0\rangle,
\charfun{x==1\land \phi}}\\
\qquad = p_2.
  \end{array}$$
  Observe that we reach the valuation $\epsilon[x\mapsto 1]$ with probability $p$ and
  $\epsilon[x\mapsto 0]$ with probability $1-p$.
%
Then, by definition, we have expectations $p_1$ and $p_1'$ such that
$\epsilon[x\mapsto 1]\models_{p_1} x==1\land \phi$,
$\epsilon[x\mapsto 0]\models_{p_1'} x==1\land \phi$
and $p_2 = p\times p_1 + (1-p)\times p_1'$.
%
Obviously, $\epsilon[x\mapsto 0]\models_{p_1'} x==1\land \phi$
is equivalent to $\epsilon\models_{p_1'} \textit{false}\land \phi$,
so $p_1'(\epsilon)==0$.
%
Similarly, $\epsilon[x\mapsto 1]\models_{p_1} x==1\land \phi$ is
equivalent to $\epsilon\models_{p_1} \phi$. Then $p_2 = p\cdot p_1$
and for all $\epsilon$ we have $\epsilon\models_{p_1} \phi$,
$\epsilon\models_{p_2} [x:=1 \pchoice{p} x:=0] (x==1 \land \phi)$ and
$p\leq \frac{p_2}{p_1}$.
% , so
% $$\phi \models_p [x:=1 \pchoice{p} x:=0] (x==1 \land \phi).$$
\end{example}
\ebjnote{it appears that we could perhaps do with equality in the definition of p-entailment.  If this is not needed in the calculus, we should perhaps strengthen.}

\begin{proposition}\label{prop:p-entailment-ordering}
$p$-Entailment is reflexive and transitive in the following sense:
\begin{enumerate}
\item $\phi\models_p \phi$ for all $p$
% \item If $\phi_1 \models_{p} \phi_2$ and $\phi_2\models_{p'} \phi_1$ then $p=p'$
\item If $\phi_1\models_{p} \phi_2$ and $\phi_2\models_{p'} \phi_3$ then $\phi_1\models_{p\times p'} \phi_3$
\end{enumerate}
\end{proposition}
\begin{proof} Let $\epsilon$ be some valuation and let $p,p',p_1,p_2,p_3\in [0,1]$.
\begin{enumerate}
\item Assume that $\epsilon\models_{p'} \phi$. Since $p\in[0,1]$, we
  have $p'\times p \leq p'$, so $\phi\models_p \phi$.
\item Assume that $\epsilon\models_{p_1} \phi_1$,
  $\epsilon\models_{p_2} \phi_2$ and\ebjnote{Having had a closer look,
    I don't think our notion of anti-symmetry holds!}
$\epsilon\models_{p_3} \phi_2$
  such that $\phi_1\models_{p} \phi_2$
  and $\phi_2\models_{p'} \phi_3$. Then $p_1\times p\leq p_2$ and
  $p_2\times p'\leq p_3$. But then $p_1\times p \times p'\leq p_2
  \times p'$, so  $p_1\times p \times p'\leq p_3$ and
  $\phi_1\models_{p\times p'} \phi_3$.
  \end{enumerate}
\end{proof}


\begin{proposition}\label{prop:p-entailment-reductions}
For any formulae $\phi_1$, $\phi_2$, and any expectation $p$ that can be expressed as a program expression:
\begin{enumerate}
    \item $\phi_1 \models_p [\, x := 1 \pchoice{p} x:=0 \,] (x==1 \land \phi_1)$ --- This property shows that an expectation of any formula $\phi_1$ can be reduced by a factor of $p$ (its expectation can be multiplied by a factor of $p$) using a simple probabilistic choice program box.
    \item $[\, x := 1 \pchoice{p} x:=0 \,] (x==1 \lor \phi_1) \models_p \phi_1 $
    \item $\phi_1 \models_p \phi_2 \quad\text{ iff }\quad \left[\,x:=1 \pchoice{p} x:=0\,\right] \left(x == 1 \land\phi_1\right) \models \phi_2\enspace,$ -- This property uses the above construction to show that p-entailment and entailment for DL-Formulas are equally expressive for this class of expectations, and within constant difference in size (the state space is doubled).
    \item  $\phi_1 \models_p \phi_2 \quad\text{ iff }\quad \phi_1 \models \left[\,x:=1 \pchoice{p} x:=0\,\right] \left(x == 1\land \phi_2\right) \enspace,$
\end{enumerate}
where $x$ is a fresh variable.
\end{proposition}

\begin{proof}
\begin{enumerate}
    \item see above
    \item todo
    \item
Assume the right hand side. Then\\
$\phi_1 \models_p [\, x := 1 \pchoice{p} x:=0 \,] (x==1 \land \phi_1)$ by Proposition \ref{prop:p-entailment-reductions}.1 and\\
$[\, x := 1 \pchoice{p} x:=0 \,] (x==1 \land \phi_1) \models_1 \phi_2$ by assumption (RHS of what we are proving) then \\
$\phi_1 \models_{1\cdot p} \phi_2$ by Proposition \ref{prop:p-entailment-ordering}.3.

\textcolor{green}{Assume that the left-hand side does not hold. Proceed by contra-positive, showing that the RHS does not hold.  Since LHS does not hold, we can apply 2.3 in the contrapositive form, and should get the conclusion (homework).}


\end{enumerate}

\end{proof}

